A vast population of wandering and merging IMBHs at cosmic noon

Massive black holes in the centers of galaxies today must have grown by several orders of magnitude from seed black holes formed at early times. Detecting a population of intermediate mass black holes (IMBHs) can provide constraints on these elusive BH seeds. Here we use the large volume, cosmological hydrodynamical simulation Astrid, which includes IMBH seeds and dynamical friction to investigate the population of IMBH seeds. Dynamical friction is largely inefficient at sinking and merging seed IMBHs at high-z. This leads to an extensive population (several hundred per galaxy) of wandering IMBHs in large halos at z~2. A small fraction of these IMBHs are detectable as HLXs, Hyper Luminous X-ray sources. Importantly, at z ~ 2, IMBHs mergers produce the peak of GW events. We find close to a million GW events in Astrid between z=2-3 involving seed IMBH mergers. These GW events (almost all detectable by LISA) at cosmic noon should provide strong constraints on IMBH seed models and their formation mechanisms. At the center of massive galaxies, where the number of IMBHs can be as high as 10-100, SMBH-IMBH pairs can form. These Intermediate mass ratio inspirals (IMRIs) and extreme mass ratio inspirals (EMRIs), will require the next generation of milli-muHz space-based GW interferometers to be detected. Large populations of IMBHs around massive black holes will probe their environments and MBH causal structure.

==> Sec2_BH_model.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Black hole models}
\label{section:BH-models}

\subsection{BH seeding}

The formation mechanism of SMBH seeds is an active research topic ~\citep[see,e.g.][for recent review]{Smith2019,Volonteri2021}. Different seeding channels have been proposed, including remnants of the first generation (Population III) stars \citep{Madau2001} creating $10 \sim 10^3 \msun$ BH seeds, direct collapse of pristine (metal-free) gas \citep{Bromm2003} and runaway collapse of nuclear star clusters \citep{Davies2011} with a higher initial seed mass ($\sim 10^4 - 10^6 \msun$).
However, these processes cannot be modelled self-consistently at the resolution of current cosmological simulations. 

In \astrid, we continue to follow the practice of seeding a BH after the formation of a sufficiently massive halo. We periodically run a Friends-of-Friends (FOF) group finder during the simulation, with a linking length of $0.2$ times the mean particle separation. Halos with a total mass and stellar mass exceeding the seeding criteria \{ $M_{\rm halo,FOF} > M_{\rm halo,thr}$; $M_{\rm *,FOF} > M_{\rm *,thr}$\} are eligible for seeding.
We apply a mass threshold value $M_{\rm halo,thr} = 5 \times 10^9 \hmsun$ and $M_{\rm *,thr} = 2 \times 10^6 \hmsun$.
The choice of $M_{\rm *,thr}$ is a conservative setting to make sure that BHs are seeded in halos with enough cold dense gas to form stars, and that there are at least some collisionless star particles in the BH neighbourhood to act as sources of dynamical friction.
The value of $M_{\rm *,thr}$ is estimated from the global $M_{\rm halo}$-$M_{\rm *}$ relation. 
Most of the FOF halos with $M_{\rm halo} > M_{\rm halo,thr}$ satisfy the $M_{\rm *,thr}$ criteria.

Considering the complex astrophysical process likely to be involved in BH seed formation, we allow haloes with the same mass to have different SMBH seeds.
Therefore, in \astrid, instead of applying a uniform seed mass for all the BHs, we probe a range of the BH seed mass $\msd$ drawn probabilistically from a power-law distribution
\begin{equation}
\label{equation:power-law}
    P(\msd ) = 
    \begin{cases}
    0 & M_{\rm sd} < M_{\rm sd,min} \\
    \mathcal{N} (M_{\rm sd})^{-n} & M_{\rm sd,min} <= M_{\rm sd} <= M_{\rm sd,max} \\
    0 & M_{\rm sd} > M_{\rm sd,max}
   \end{cases}
\end{equation}
where $\mathcal{N}$ is the normalization factor.
We set $M_{\rm sd,min} = 3 \times 10^4 \hmsun$, $M_{\rm sd,max} = 3 \times 10^5 \hmsun$, and a power-law index $n = -1$. 
In Section \ref{subsection3.4}, we investigate the effect of $M_{\rm sd}$ on BH growth. 

For each halo that satisfies the seeding criteria but does not already contain at least one SMBH particle, we convert the densest gas particle into a BH particle. 
The newborn BH particle inherits the position and velocity of its parent gas particle. 
The intrinsic mass of BH ($M_{\rm BH}$ hereafter) seeds are initially at $M_{\rm sd}$ (as a subgrid mass). However, we preserve in a separate mass variable the parent particle mass, representing a subgrid gas reservoir around the SMBH.
Neighbouring gas particles are swallowed once (Eddington-limited) accretion has allowed $M_{\rm BH}$ to grow beyond the initial parent particle mass (i.e., once it depletes the gas reservoir of the parent gas particle).


%-------------------------------------------
\subsection{BH dynamics and mergers}
\label{subsection:BH dynamics}

A common approach applied in cosmological simulations is to anchor the BH at the halo potential minimum by forcefully repositioning the BH particle to the local (within the SPH kernel) potential minimum at every active timestep. While this method is effective at stabilizing the BH in the halo centre, it means that the BH trajectory is discontinuous and the BH velocity is ill-defined. In addition, should two galaxies pass close enough to each other, a BH merger can result immediately even though they are not gravitationally bound.

We instead use a sub-grid dynamical friction model \citep{Chen2021} to account for the unresolved frictional force exerted by the surrounding collisionless matter (stars and stellar-mass black holes) on SMBH dynamics. In this model, SMBHs gradually sink to the galaxy centre, as their relative velocity is dissipated by dynamical friction. 
Moreover, we can make a more physical prediction for BH mergers by calculating whether the (now well-defined) relative velocities of two SMBHs allow them to be gravitationally bound.
The validation of our dynamical friction model in cosmological simulations was performed in \cite{Chen2021}. In this section, we briefly review the BH dynamics.

%-------------------------------------------
\subsubsection{Dynamical friction}
\label{subsubsection:dynamic-friction}

When an SMBH moves through an extended medium composed of collisionless particles with smaller mass, it experiences a drag force. The source of this force is the gravitational wake from perturbing the particles in the surrounding medium \citep{Chandrasekhar1943}. 
This drag force is called dynamical friction and it effectively transfers energy and momentum from the SMBH to surrounding particles, thus dissipating the SMBH momentum relative to its surroundings.
Dynamical friction causes the SMBH orbit to decay towards the centre of massive galaxies \citep[e.g.][]{Governato1994,Kazantzidis2005} and also stabilizes the BH motion at the centre of the galaxy.

We estimate dynamical friction on SMBHs using Eq. 8.3 of \cite{Binney2008}: 
\begin{equation}
\label{eq:df_full}
    \mathbf{F}_{\rm DF} = -16\pi^2 G^2 M_{\rm BH}^2 m_{a} \;\text{log}(\Lambda) \frac{\mathbf{v}_{\rm BH}}{v_{\rm BH}^3} \int_0^{v_{\rm BH}} dv_a v_a^2 f(v_a),
\end{equation}
$M_{\rm BH}$ is the BH mass, $\textbf{v}_{\rm BH}$ is the BH velocity relative to its surrounding medium, $m_a$ and $v_a$ are the masses and velocities of the particles surrounding the BH, and $\text{log}(\Lambda)=\text{log}(b_{\rm max}/b_{\rm min})$ is the Coulomb logarithm that accounts for the effective range of the friction between the specified $b_{\rm min}$ and $b_{\rm max}$. 
$f(v_a)$ in Eq.~\ref{eq:df_full} is the velocity distribution of the surrounding collisionless particles including both stars and dark matter. 
Here we have assumed an isotropic velocity distribution of the particles surrounding the BH so that we are left with a 1D integration. 

In \astrid, the BH seed mass extends down to $3\times 10^4 \hmsun$, which is one order of magnitude smaller than the stellar particle mass. 
At this $\mbh$ regime, the dynamical friction of BH is underestimated due to the limited mass resolution of the star particles, and so the dynamics of the seed BH would be unstable without repositioning.
As a compromise, we replace the $\mbh$ in Eq.~\ref{eq:df_full} with $M_{\rm dyn}$. This temporarily boosts the BH dynamic mass for BHs near the seed mass, stabilizing their motion during the early post-seeding evolution.
We will further discuss this implementation in Section~ \ref{subsubsection:DynamicBHMass}.


We approximate $f(v_a)$ by the Maxwellian distribution \citep[as, e.g.][]{Binney2008}, and account for the neighbouring collisionless particles up to the range of the SPH kernel of the BH particle \citep[see,][for more details]{Chen2021}. 
Eq.~\ref{eq:df_full} reduces to
\begin{equation}
    \label{eq:H14}
    \mathbf{F}_{\rm DF} = -4\pi \rho_{\rm sph} \left(\frac{GM_{\rm dyn}}{v_{\rm BH}}\right)^2  \;\text{log}(\Lambda) \mathcal{F}\left(\frac{v_{\rm BH}}{\sigma_v}\right) \frac{\bf{v}_{\rm BH}}{v_{\rm BH}}.
\end{equation}
Here $\rho_{\rm sph}$ is the density of dark matter and star particles within the SPH kernel. 
The function $\mathcal{F}$, defined as
\begin{equation}
    \label{eq:fx}
    \mathcal{F}(x) =  \text{erf}(x)-\frac{2x}{\sqrt{\pi}} e^{-x^2}, \;
    x=\frac{v_{\rm BH}}{\sigma_v}
\end{equation}
is the result of analytically integrating the Maxwellian distribution. $\sigma_v$ is the velocity dispersion of the surrounding particles.
The Coulomb logarithm $\Lambda$ is calculated with
\begin{equation}
    \Lambda = \frac{b_{\rm max}}{(GM_{\rm dyn})/v_{\rm BH}^2}
\end{equation}
where $b_{\rm max} = 20\text{ kpc}$ is an ad hoc choice for the maximum physical range to account for the frictional force. 

%-------------------------------------------
\subsubsection{Gas Drag}
\label{subsubsection:gas-drag}
In addition to the dynamical friction from the collisionless particles (dark matter and stars), we also add a drag force on the BH from the surrounding gas particle, with
\begin{equation}
\label{eq:drag}
    \mathbf{a}_{\rm drag} = (\mathbf{v}_{\rm gas}-\mathbf{v}_{\rm BH})\dot{M}_{\rm BH}/M_{\rm BH}
\end{equation}
This term is motivated by the BH gaining momentum from the surrounding gas continuously, bringing the sinking of the BH with respect to the gas.
It is a subdominant factor compared to the dynamical friction exerted by collisionless particles \citep{Chen2021}.


%-------------------------------------------
\subsubsection{Dynamic mass of BH}
\label{subsubsection:DynamicBHMass}


In \astrid, the minimal BH seed mass is $3\times 10^4 \hmsun$, orders of magnitude smaller than the stellar and DM particle masses.
Such a small BH mass relative to the surrounding particles causes noisy gravitational forces (dynamical heating) around the BH and thus instability in the BH motion.  Moreover, as shown in some previous works~\citep[e.g.][]{Tremmel2015,Pfister2019}, it is challenging to effectively model dynamical friction in a sub-grid fashion when $M_{\rm BH}/M_{\rm DM} \ll 1$. 


Following \cite{Chen2021}, we introduce another BH mass tracer, the dynamical mass $M_{\rm dyn}$, to account for the force calculation of BH (including the gravitational force and dynamical friction).  
Note that we still use the intrinsic BH mass $M_{\rm BH}$ to account for the BH accretion and AGN feedback. 
When a new BH is seeded, we initialize the corresponding $M_{\rm dyn} = M_{\rm dyn,seed} = 10^7 \hmsun$, which is about $1.5 M_{\rm DM}$. 
\cite{Chen2021} showed that this alleviates dynamic heating and stabilizes the BH motion in the early growth phase.
$M_{\rm dyn}$ is kept at its seeding value until $M_{\rm BH}>M_{\rm dyn,seed}$.
After that, $M_{\rm dyn}$ grows following the BH mass accretion.


The boost of the initial $M_{\rm dyn}$ may overestimate the dynamical friction for small BHs and the resultant sinking time scale will be shortened by a factor of $\sim M_{\rm BH}/M_{\rm dyn}$ compared to the no-boost case.
On the other hand, it is also possible that the BH sinking time scale estimated in our simulation in the no-boost case could overestimate the true sinking time, as the high-density stellar bulges are not fully resolved \citep[e.g.][]{Antonini2012,Dosopoulou2017,Biernacki2017}.
Therefore, boosting the initial $M_{\rm dyn}$ seems a reasonable compromise to model the dynamics of small mass BHs while also alleviating the noisy perturbation of dynamic heating brought by the limit of resolution. 
Note that even if our dynamic friction implementation overestimates the force, it still provides a substantially more conservative estimation of BH sinking than the common model where SMBHs are aggressively repositioned to the potential minimum.

%-------------------------------------------
\subsubsection{BH Mergers}
\label{subsubsection:BH-merger}

In \astrid, BHs have a well-defined dissipative velocity subject to dynamic friction, allowing us to impose a more physical criterion for BH mergers based on the relative velocities and accelerations of merging SMBH pairs.
Following \cite{Bellovary2011} and \cite{Tremmel2017}, we check whether two nearby BHs are gravitationally bound using the criteria
\begin{equation}
\label{equation:merger}
    \begin{cases}
    |\bf{\Delta r}| < 2 \epsilon_{\rm g} \\
    \frac{1}{2}|\bf{\Delta v}|^2 < \bf{\Delta a} \bf{\Delta r} \,.\\
   \end{cases}
\end{equation}
Here $\epsilon_{\rm g} = 1.5 \hkpc$ is the gravitational softening length.
We set the merging distance based on $\epsilon_{\rm g}$ as BH dynamics below this distance are not spatially resolved.
$\bf{\Delta a}$,$\bf{\Delta v}$ and $\bf{\Delta r}$ denote the relative acceleration, velocity and position of the BH pair, respectively. 
Note that this expression is not strictly the total energy of the BH pair, but an approximation to the kinetic energy and the work needed to get the BH to merge. 

The BH merging criteria applied in \astrid is an improvement compared with many cosmological simulations where BH dynamics are modelled with repositioning.
In simulations with BH repositioning, the distance between the two BHs is essentially the only merging criteria. It might spuriously merge two BHs with high relative velocities when in reality they are not gravitationally bound and should not merge yet (or may never merge). 
Some cosmological simulations \citep[e.g.][]{Schaye2015,Dave2019-simba} also apply gravitational binding or escape velocity criteria for a BH merger. However, in those cases, the BHs still do not have a well-defined velocity and sinking time.

Moreover, as the BH pairs in \astrid now have well-defined orbits down to the numerical merger time, we can make use of the binary separation and eccentricity measured at the time of numerical merger as the initial conditions when post-processing BH mergers at sub-resolution scale, without having to assume a constant value as in \cite{Kelley2017}.
We will address this further in our follow up work \citep{Chen2021b}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{BH accretion and feedback}

We model BH growth and AGN feedback as in the \bluetides~simulation. 
BHs are allowed to grow by accreting mass from nearby gas particles.
The gas accretion rate onto the BH is estimated via the Bondi-Hoyle-Lyttleton-like prescription applied to the smoothed properties of the $112$ gas particles within the SPH kernel of the BH:
\begin{equation}
\label{equation:Bondi}
    \dot{M}_{\rm B} = \frac{4 \pi \alpha G^2 M_{\rm BH}^2 \rho}{(c^2_s+v_{\rm rel}^2)^{3/2}}
\end{equation}
$c_s$ and $\rho$ are the local sound speed and density of gas, $v_{\rm rel}$ is the relative velocity of the BH with respect to the nearby gas and $\alpha = 100$ is a dimensionless fudge parameter to account for the underestimation of the accretion rate due to the unresolved cold and hot phase of the subgrid interstellar medium nearby.
Note that hydrodynamically decoupled wind particles are not included in the density calculation of Eq.~\ref{equation:Bondi}.

We allow for short periods of super-Eddington accretion in the simulation, but limit the accretion rate to $2$ times the Eddington accretion rate
\begin{equation}
\label{equation:Meddington}
    \dot{M}_{\rm Edd} = \frac{4 \pi G M_{\rm BH} m_p}{\eta \sigma_{T} c}\,.
\end{equation}
$m_p$ is the proton mass, $\sigma_T$ the Thompson cross section, c the speed of light, and $\eta=0.1$ the radiative efficiency of the accretion flow onto the BH.

In summary, the total BH accretion rate in the \astrid simulation is:
\begin{equation}
    \dot{M}_{\rm BH} = {\rm Min} (\dot{M}_{\rm B}, 2\dot{M}_{\rm Edd})
\end{equation}

Numerically, the physical BH mass, $\mbh$, grows continuously with time, while we separately track the BH dynamic mass by stochastic accretion of nearby gas particles with a probability that statistically satisfies mass conservation. Given that $M_{\rm dyn}$ is temporarily boosted (and initially fixed) for the new-born BH particles for gravity and dynamical friction calculation, we use a separate mass tracer $M_{\rm trace}$ to perform gas accretion when $\mbh < M_{\rm dyn,seed}$. This term is initialized as the parent particle mass that spawns the BH, and traces $\mbh$ with stochastic gas accretion until $\mbh >= M_{\rm dyn,seed}$. After that, $M_{\rm dyn}$ grows following $\mbh$ by swallowing gas.

To ensure stable accretion, the timestep of the BH particle is set not by the acceleration dynamics, but by being $2$ times longer than the smallest timestep found amongst the gas particles within its density kernel. 

AGN thermal feedback is implemented as follows.
The SMBH is assumed to radiate with a bolometric luminosity $L_{\rm Bol}$ proportional to the accretion rate $\dot{M}_{\rm BH}$:
\begin{equation}
\label{equation:Lbol}
    L_{\rm Bol} = \eta \dot{M}_{\rm BH} c^2
\end{equation}
with $\eta = 0.1$ being the mass-to-light conversion efficiency in an accretion disk according to \cite{Shakura1973}.
5\% of the radiated energy is thermally coupled to the surrounding gas that resides within twice the radius of the SPH smoothing kernel of the BH particle. 

The AGN feedback energy is isotropically imparted to the nearby gas particles, distributing the energy among them according to the SPH kernel.
Gas particles that are heated by AGN feedback dissipate the energy in different channels depending on their thermal properties.
Non star-forming gas cools as normal, while star-forming gas heated by the SMBH relax to the temperature corresponding to the effective equation of state for star-forming \citep[c.f.][]{2003MNRAS.339..289S}, on a time scale determined by the cooling time. Note that star-forming gas heated by other means cools to the effective equation of state on the longer relaxation timescale.

%-------------------------------------------
\subsection{BH catalogs in \astrid}

For every time step in the simulation, we log the full physical state of all the active BH particles, including the thermal states (density, entropy), dynamics (position, velocity, acceleration from gravity, dynamical friction, gas drag), growth state (mass, accretion rate, accretion of gas and BHs), neighbour information (number of surrounding particles, local velocity dispersion) etc, to a separate catalogue.
This high time resolution BH catalogue allows us to follow the detailed growth history of all BHs in the simulation, build the merger trees of BHs, trace the trajectory of BH merger events down to $\kpc$ scale and allow post-processing of BH mergers at sub-resolution scale based on the orbits of BHs. 

